TraceCaps: A Capsule-based Neural Network for Semantic Segmentation

In this paper, we propose a capsule-based neural network model to solve the semantic segmentation problem. By taking advantage of the extractable part-whole dependencies available in capsule layers, we derive the probabilities of the class labels for individual capsules through a recursive, layer-by-layer procedure. We model this procedure as a traceback pipeline and take it as a central piece to build an end-to-end segmentation network. Under the proposed framework, image-level class labels and object boundaries are jointly sought in an explicit manner, which poses a significant advantage over the state-of-the-art fully convolutional network (FCN) solutions. With the capability to extracted part-whole information, our traceback pipeline can potentially be utilized as the building blocks to design interpretable neural networks. Experiments conducted on modified MNIST and neuroimages demonstrate that our model considerably enhance the segmentation performance compared to the leading FCN variants.

==> conclusion_tao.tex <==
\section{Discussion and Related Work}
Since the inception of the first FCN model, FCN variants have become
the most popular solutions for semantic segmentation. Compared with
traditional non-deep learning techniques as well as patch-based CNN
solutions, the efficacy of FCNs should be attributed, in large part,
to their capability to process information from various spatial
scales.

\paragraph{FCN models} While powerful, FCNs also have some inherent
limitations. Originated from CNNs, FCNs tend to lose precise spatial
information along the pooling operations/layers, and inconsistent
pixel labelings can be resulted from the limited receptive field at
each neuron. A number of approaches have explored to add the
contextual information back to the CNN component. Conditional Random
Fields (CRFs) based solutions \citep{chen2014crf,chen2018deeplab}
refine the final segmentation results with a post-processing stage to
boost its ability to capture fine-grained details. Dilated
convolutions \citep{yu2015dilate,yu2017dilated} are utilized to take
advantage of the fact that the receptive fields of systematic dilation
can be expanded exponentially without losing resolution. Fusion of
global features extracted at lower layers and local features from
higher layers through skip connections have also been well studied
\citep{long2015fully,ronneberger2015unet}. To produce segmentation
results with certain shape constraints,
\citep{ravishankar2017shape,chen2013shape} integrate shape priors into
existing deep learning framework with shape-based loss terms. New
models have emerged in the past {\color{red} two years} or so, such as
multi-resolution fusion by RefineNet \citep{lin2017refinenet}, pyramid
pooling module in PSPNet \citep{zhao2017pyramid}, Clusternet
\citep{lalonde2018clusternet}, atrous convolution and fully connected
CRFs \citep{zhang2018exfuse}, Y-Net \citep{mehta2018net},
{\color{red}HRNet \citep{sun2019high}, Panoptic-deeplab
  \citep{cheng2020panoptic}, and models trained with self-training
  \citep{zoph2020rethinking}}.


% Zhenli Zhang, Xiangyu Zhang, Chao Peng, Dazhi Cheng, and Jian
% Sun. Exfuse: Enhancing feature fusion for semantic
% segmentation. arXiv preprint arXiv:1804.03821, 2018.

\paragraph{Capsules, supervised and unsupervised capsulet nets}
The history of the notion of capsules can be dated back to
\citep{hinton1981capsule}, in which the author proposed to describe an
object over the viewpoint-invariant spatial relationships between the
object and its parts. This model should be regarded as the first
theoretical prototype of the recent capsule nets
{\color{red}\citep{hinton2017nips,hinton2018ICLR,hinton2019Nips}}. \cite{zemel1990traffic}
added probability components into this prototype and encoded both
probabilities and viewpoint-invariance in a fully-connected neural
network. The instantiation parameters of Zemel’s model were
hand-crafted from input data.

The issue of how to initialize instantiation parameters was partially
addressed in \citep{hinton2011autoencoder}, but their model requires
transformation matrices to be input externally. Regarding the routing
algorithms, \cite{zemel1990traffic} introduced the notion that an
object can be activated by combining the predictions from its parts,
which was materialized as an averaging operation in
\citep{hinton2011autoencoder}.  \cite{hinton2017nips,hinton2018ICLR}
took a step forward and resorted to routing-by-agreement algorithms to
simultaneously activate objects and set up part-whole relationships.

{\color{red} Adapting from the ideas of capsule initiation
  % in \citep{hinton2011autoencoder}
  and the routing mechanism in supervised capsule nets, 
  % \citep{hinton2018ICLR},
  unsupervised capsule nets
  \citep{hinton2019Nips} leverage set transformer \citep{lee2019ICLR}
  to infer whole-part relationships.

  In addition to inner product
  \citep{hinton2017nips} and Gaussian distribution
  \citep{hinton2018ICLR} based routing mechanisms,

  other routing methods were proposed, including attention-based routing
  procedure \citep{choi2019attention,duarte2019capsulevos}, distance
  measures based method \citep{lenssen2018group}, and weighted kernel
  density estimation based method
  \citep{zhang2018fast}. \cite{mcIntosh2020vt} introduced
  visual-textual routing mechanism to jointly learned video and text
  capsules for video segmentation.  \cite{lalonde2019encoding}
  proposed a routing sigmoid function to aid the encoding of
  high-level visual object attributes, which helps explain of lung
  cancer predictions with language similar to human-experts. Besides,
  capsule networks have also been applied extensively to such areas as
  text classification \citep{zhao2018investigating}, action detection
  \citep{duarte2018video}, visual question answering
  \citep{zhou2019dynamic} and medical image analysis
  \citep{lalonde2020diagnosing,afshar2018brain,iesmantas2018convolutional,mobiny2019automated,pal2018capsdemm}.}

\paragraph{Capsule-based segmentation solutions}

To the best our knowledge, {\color{red}two capsule-based models
  \citep{lalonde2018capsules, bonheur2019matwo}} has been proposed for
the segmentation task. The {\color{red}object segmentation model
  (\textit{SegCaps})} \citep{lalonde2018capsules} made two
modifications to the original dynamic routing algorithm, such that the
number of parameters is greatly reduced, which enables the model to
operate on large images sizes. Deconvolutional capsule layers were
devised and appended directly to convolutional capsule layers to
restore the original resolution. Similar to FCNs, this model utilizes
skip connections to integrate contextual information from different
spatial scales. {\color{red}\cite{bonheur2019matwo} introduced
  \textit{Matwo-CapsNet}, a U-shaped (similar to U-Net) semantic
  segmentation model enabled by a new type of capsule encoding pose
  and appearance information and Dual Routing combing these two kinds
  of information}. Our TraceCaps, however, is designed under a
different paradigm. Taking the extractable part-whole information as
the foundation, label assignments in TraceCaps are explicit,
interpretable, and mathematically well-grounded. The decoder of our
model is much simpler than that of \citep{lalonde2018capsules} model,
with no trainable parameters (up to deconvolution layers) and no
capsule-wise routing needed. Because of the analytical derivations,
our model has great potential to be applied to many other
applications, including object localization, detection and
visualization of heap maps. {\color{red}Although Matwo-CapsNet
  \citep{bonheur2019matwo} was claimed to perform much better than
  SegCaps, performances of both Matwo-CapsNet and SegCaps
  \citep{lalonde2018capsules, bonheur2019matwo} were on a par with
  that of the state-of-the-art model (i.e. U-Net). As a comparison,
  TraceCaps considerably enhances the segmentation performance of
  U-Net in our experiments.}


\paragraph{From capsule-based recognition to capsule-based segmentation and beyond}
Capsule nets have an assumption in
  their constructions: \textquotedblleft at each location in the image, there is at
  most one instance of the type of entity that a capsule represents.\textquotedblright \citep{hinton2017nips}. 
  Essentially, capsule nets, including the
  internal part-whole relationships, are built on concrete, physical
  object instances. With this assumption, capsule nets perform well
  when there is at most one instance of a category in the image, such
  as on MNIST and smallNORB \citep{lecun2004learning}. For the image
  data that have multiple instances of same classes, capsule nets have
  no guarantee to outperform CNNs in recognition accuracy.

The traceback pipeline in our TraceCaps does not rely
  on the this one-instance assumption. However, the current version
  TraceCaps is designed based on the capsule nets, where the margin
  loss is specified with outputs of the class capsule layer. The
  inability of capsule nets in handling multi-instance-same-class
  cases also limits the capacity of our segmentation model, for
  certain type of dataset. Regarding the remedies, we believe efforts
  can be push forward along three fronts. The first one would rely on
  the continued development of capsule and capsule nets to overcome
  their limitations. The second possibility would be designing
  traceback solutions that can circumvent the multi-instance
  constraint. For example, if the class capsule layer can somehow be
  removed from the traceback pipeline, potentially we could
  accommodate multiple instances of the same category, starting at a
  convolutional capsule layer. The third group of remedies could be
  developed along pre-processing direction. For example, object
  detection can be carried out first, followed by TraceCaps to
  generate accuracy segmentations within individual regions.

\bigskip

%\textcolor{red}{To sum up, we propose a capsule-based segmentation
%  solution in this paper. By taking advantage of the part-whole
%  relationship in capsule-based networks and build our model on top of
%  CapsNets. With object recognition is specifically designed and
%  formulated as an integral component, our CapSegNet integrates
%  multi-scale semantical and location information in an explicit
%  way. Experimental results demonstrate our model outperforms U-Net in
%  several datasets, and the improvements are made in many aspects
%  including segmentation accuracy and label consistency.}


==> implementation.tex <==
%\section{Implementation}
%
%\subsection{Architecture}
%There are three components in the TbCapsNet. The first one is the feature
%engineering component which prepares the features needed by the capsule layers.
%Usually the component consists of regular convolutional layers adapted
%from classical ConvNets such as VGG-16 or ResNet-101. The second component is 
%capsule layers and traceback layers. Capsule layers can be combinations of one primary 
%capsule layer, several optional convolutional capsule layers, and one class capsule layer. 
%Traceback layers use derivation in the previous sections to infer the class labels for each
%capsules in the primary capsule layer. The third component restores the 
%original resolution by interpolating the label map computed in the traceback layers.
%Exemplified layer implementation for the component are based on deconvolution,  
%atrous convolution, or bilinear interpolation. 
%
%Current  traceback layer assigns the class labels for the last capsule layer (i.e. the 
%$L-1$ layer in Fig. \ref{fig:generalcaps}). To simplify the derivation, we use $p(m)$
%to denote the probability of a capsule of type $m \in \mathcal{T}^{L-1}$ at the
%position $(i, j)$ in the \textit{PrimaryCapsules} layer and $c_{mk}$
%to denote its coupling coefficient with a class capsule
%$\mathcal{C}_{k}$ (Fig. \ref{fig:arch}). And so Equation \ref{eq:segclass} becomes
%
%\begin{equation}
%\begin{aligned}
%  p(\mathcal{C}_{k}) &= \sum_{m \in T^{L-1}} p(m, k) = \sum_{m \in T^{L-1}} p(m)p(k|m) \\
%                                              &= \sum_{m \in T^{L-1}}p(m)c_{mk}.
% \end{aligned}
%\end{equation} 



%The detailed encoder-decoder configuration of the model is illustrated
%in Fig. \ref{fig:arch}. For the encoder, all the layers in CapsNets
%\citep{hinton2017nips} except reconstruction part are applied. This is
%a shallow architecture consisting of one convolutional layer, one
%primary capsule layer and a class capsule layer. The first layer is a
%regular convolutional layer with 256 $9\times 9$ kernels converting
%pixels to feature maps, which is then feed into a modified convolution
%layer named \textit{PrimaryCapsules}. The \textit{PrimaryCapsules}
%performs convolutional operations with $8\times 32$ kernels. Each 8
%layers of the resulted neurons are then grouped to form 32-layer 8-D
%capsules. The class capsules take the capsules in
%\textit{PrimaryCapsules} as input and apply a transformation matrix to
%convert a 8-D capsule to a 16-D capsule for each class.

% As the network in \citep{hinton2017nips}, the length of the
% activation vector represents the probability with which the capsule
% exists and the orientation of the vector represents its
% instantiation parameters. The total input of a capsule is calculated
% through the weighted sum of all the predictions from its children in
% the previous layer
%
%\begin{equation}
%	\textbf{s}_{j_n^{l+1}} = \sum_{i \in ch(j)}  c_{i_m^l j_n^{l+1}} \textbf{v}_{(j_n^{l+1}|i_m^l)},
%\end{equation}
%
%The input is normalized to 1 by a squashing function
%
%\begin{equation}
%	\textbf{u}_{j_n^{l+1}} = \frac{\Vert \textbf{s}_{j_n^{l+1}}\Vert ^{2}}{1 + \Vert \textbf{s}_{j_n^{l+1}} \Vert ^{2}} \frac{\textbf{s}_{j_n^{l+1}}}{\Vert \textbf{s}_{j_n^{l+1}} \Vert }
%\end{equation}




%With the equation, a class map for each predefined class with the same
%size as the \textit{PrimaryCapsules} can be calculated. Since the size
%of those class maps are smaller than that of the input image,
%upsampling operations are needed to restore the original image
%size. Actually just like the encoder of the FCN models, there exists
%many choices for the upsampling operations. After experiments, we
%concluded that the design following the idea of the decoder of U-Net
%achieves the best performances. And thus each layer in the decoder is
%upsampled with the deconvolutiuon after they are concatenated with the
%corresponding encoder layer.

%% should we mention why?

%\subsection{Loss Function}
%The loss function is a weighted sum of the margin loss over the class
%capsules \citep{hinton2017nips} and pixel-wise softmax cross-entropy 
%loss over the final feature map. 
%The margin loss strives to increase the probabilities of class capsules that 
%exist in the input data. For each predefined class, there exists a term $L_k$ in the
%margin loss
%\begin{equation}
%\begin{aligned}
%  L_k = \ & T_k \ max(0, m^{+}  - p(\textbf{v}))^2 \ \\ & + \lambda (1-T^k)\ max(0, m^{+}  - p(\textbf{v}) )^2
%\end{aligned}
%\end{equation}
%
%where $m^{+} =0.9$, $m^{-} =0.1$, and $\lambda =0.5$. The $T_k=1$ when
%a class $k$ is present in the mask and $T_k=0$ otherwise.
%
%The margin loss plays a key role in training of the model because it
%is the driving force for the initiation and convergence of the capsule layers
%in the model. While the cross-entropy loss handles the boundary localization
%in semantic segmentation, the margin loss is responsible for the
%object recognition. As a result, the weights ratio between margin loss
%and softmax loss in the combined loss function is an important
%hyper-parameter to tune the performance of our models.



%AdamOptimizer learning rate
%loss function








==> related.tex <==
\section{Related work}
Semantic segmentation is a problem that requires the % balanced
integration of local and global information from multiple scales.
% of information from various spatial scales. It also implies balancing local and global information.
% On the one hand, fine-grained or local information is crucial to
% achieve good pixel-level accuracy. On the other hand, it is also
% important to integrate information from the global context of the
% image to be able to resolve local ambiguities.  Vanilla CNNs
% struggle with this balance. Pooling layers, which allow the networks
% to achieve some degree of spatial invariance and keep computational
% cost at bay, dispose of the global context information. Even purely
% CNNs – without pooling layers – are limited since the receptive
% field of their units can only grow linearly with the number of
% layers.
\paragraph{FCN models} Originated from CNNs, FCN models tend to lose precise spatial
information along the pooling operations/layers, and inconsistent
pixel labelings can be resulted from the limited receptive field at
each neuron. A number of approaches
% approaches under the FCN framework
have explored to add the contextual information back to the CNN
component. Conditional Random Fields (CRFs) based solutions
\cite{chen2014crf,chen2018deeplab} refine the final segmentation results with a
post-processing stage to boost its ability to capture fine-grained
details. Dilated convolutions \cite{yu2015dilate,yu2017dilated} are utilized to take advantage of
the fact that the receptive fields of systematic dilation can be
expanded exponentially without losing resolution.
% Multi-scale prediction is another possible way to integrate context
% knowledge.
Fusion of global features extracted at lower layers and local
features from higher layers through skip connections have also been
well stuided \citep{long2015fully,ronneberger2015unet}. To produce
segmentation results with certain shape constraints,
\citep{ravishankar2017shape,chen2013shape} integrate shape priors
into existing deep learning framework with shape-based loss terms.

%DeepLab \cite{} and ENet \cite{} use combinations of dilated
%convolutions with increasing dilation rates to have wider receptive fields
%without overaly downsampling the feature maps. 
% Many approaches can be taken to make CNNs aware of that global
% information: refinement as a post-processing step with Conditional
% Random Fields (CRFs), dilated convolutions, multi-scale aggregation,
% or even defer the context modeling to another kind of deep networks
% such as RNNs.
%In order to remedy the defect, 
%\citep{ravishankar2017shape, chen2013shape} attempts to learn shape
%priors and impose them into existing deep learning frameworks.
%In \citep{chen2014crf}, the final segmentation results from the deep
%learning classification framework is refined by a conditional random
%field (CRF) to capture more fine details.
%Based on the fact that the
%receptive fields of systematic dilation can be expanded exponentially
%without losing resolution, \citet{yu2015dilate} introduces a novel CNN
%architecture, which leverage the dilated convolution to aggregate
%multi-scale context. \citet{chen2016combining} feeds 2D images of
%different scales to a sequence of FCN submodules, which actually is a
%simulation of the mechanism human experts use to comprehend
%multi-scale information.
%Although these methods outperform the
%performance of demanding benchmarks, they does not disentangle the key
%factors which hinder the FCN models to better achieve the balance
%between global and local information.

%Currently, the most successful state-of-the-art deep
%learning techniques for semantic segmentation stem from a common
%forerunner: the Fully Convolutional Network (FCN) by Long et
%al. [65].
%The insight of that approach was
%FCNs take advantage of existing CNNs as powerful visual models that
%are able to learn hierarchies of features.
% They transformed those existing and well-known classification models – AlexNet [14], VGG (16-layer net)
% [15], GoogLeNet [16], and ResNet [17] – into fully convolutional ones
% by replacing the fully connected layers with convolutional ones to
% output spatial maps instead of classification scores.
% Those maps are upsampled using fractionally strided convolutions (also named
% deconvolutions [90] [91]) to produce dense per-pixel labeled
% outputs. This work is considered a milestone since it showed how CNNs
% can be trained end-to-end for this problem, efficiently learning how
% to make dense predictions for semantic segmentation with inputs of
% arbitrary sizes.
%This approach achieved a significant improvement in
%segmentation accuracy over traditional methods on standard datasets
%like PASCAL VOC, while preserving efficiency at inference.
% For all those reasons, and other significant contributions, the FCN
% is the cornerstone of deep learning applied to semantic
% segmentation. The convolutionalization process is shown in Figure 7.

%Despite the power and flexibility of the FCN model, it still lacks
%various features which hinder its application to certain problems and
%%situations: its inherent spatial invariance does not take into
%account useful global context information,
%no instance-awareness is
%present by default, efficiency is still far from real-time execution
%at high resolutions, and it is not completely suited for
%unstructured data such as 3D point clouds or models.


\paragraph{Capsules and Capsule Networks} Hinton 1981 proposed to describe an object over the viewpoint-invariant spatial relationships between the canonical reference frame of the object and the reference frame of its parts. And furthermore it is also suggested implementing the description in a parallel network. This should be the theoretical prototype of the current capsule networks \citep{hinton2017nips,hinton2018ICLR}. \cite{zemel1990traffic} involves probability into the prototype and implemented it in a connectionist network. In the meantime,  the issue is raised converting a input image into initial input features of the model. Although the issue was resolved in \citep{hinton2011autoencoder}, it requires transformation matrices to be specified as input parameters.  \cite{zemel1990traffic} suggested the idea that an object can be activated by combining the predictions from its parts, which was materialized as average operation in \citep{hinton2011autoencoder} .\cite{hinton2017nips,hinton2018ICLR} took a step forward and resorted to routing-by-agreement algorithms to activate objects and set up part-whole relationships simultaneously. The first capsule segmentation model \citep{lalonde2018capsules} introduced deconvolutional capsule layers, which are appended directly to convolutional capsule layers to restore the original resolution.  Similar to FCN and its variants, it uses skip connections to add the contextual information back.



%To exploit the inter-slice contexts in segmentation of 3D medical images, joint FCN  and 
%recurrent neural network models are proposed to enhance accuracy of segmentation 
%\citep{chen2016combining, Tseng2017joint, chen2017accurate}.

